Diversity-aware Multi-Video Summarization

Most video summarization approaches have focused on extracting a summary from a single video; we propose an unsupervised framework for summarizing a collection of videos. We observe that each video in the collection may contain some information that other videos do not have, and thus exploring the underlying complementarity could be beneficial in creating a diverse informative summary. We develop a novel diversity-aware sparse optimization method for multi-video summarization by exploring the complementarity within the videos. Our approach extracts a multi-video summary which is both interesting and representative in describing the whole video collection. To efficiently solve our optimization problem, we develop an alternating minimization algorithm that minimizes the overall objective function with respect to one video at a time while fixing the other videos. Moreover, we introduce a new benchmark dataset, Tour20, that contains 140 videos with multiple human created summaries, which were acquired in a controlled experiment. Finally, by extensive experiments on the new Tour20 dataset and several other multi-view datasets, we show that the proposed approach clearly outperforms the state-of-the-art methods on the two problems-topic-oriented video summarization and multi-view video summarization in a camera network.

==> MathDetails.tex <==
\begin{equation}
	\begin{gathered}
		\label{eq:singlevideo}
		\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda^{\it{(v)}}_s\lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\
		s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1},\ {\bf{Z^{(\it{v})}}} \in \mathbb{R}^{n_v\times n_v}
	\end{gathered}
%	\vspace{-2mm}
\end{equation}  

\begin{equation}
\begin{gathered}
\label{eq:naivemultivideo}
\min_{\bf{Z^{(1)}},\bf{Z^{(2)}},\cdots,\bm{Z^{({m})}}} \ \sum_{v=1}^{m}\lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \sum_{v=1}^{m} \lambda^{\it{(v)}}_s\lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1},\ {\bf{Z^{(\it{v})}}} \in \mathbb{R}^{n_v\times n_v},\ \forall \ 1 \leq \it{v} \leq m	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:diversity}
{f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})} = \frac{1}{\it{n}_{v}n_{w}}\sum_{i=1}^{n_v}\sum_{j=1}^{n_w}\lVert{\bf{Z^{(\it{v})}_{\it{i}}} \rVert}_{2,1}{\bf{C_{\it{ij}}}}\lVert{\bf{Z^{(\it{w})}_{\it{j}}} \rVert}_{2,1}
\end{gathered}
%\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:diversityW}
{\bf{W^{\it{(vw)}}_{\it{ii}}}} = \frac{1}{\it{n}_{v}n_{w}}\sum_{j=1}^{n_w}{\bf{C_{\it{ij}}}}\lVert{\bf{Z^{(\it{w})}_{\it{j}}} \rVert}_{2,1}
\end{gathered}
%\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:diversityfinal}
{f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})} = \sum_{i=1}^{n_v}\sum_{j=1}^{n_w}\lVert{\bf{Z^{(\it{v})}_{\it{i}}} \rVert}_{2,1}{\bf{C_{\it{ij}}}}\lVert{\bf{Z^{(\it{w})}_{\it{j}}} \rVert}_{2,1}=\lVert{\bf{W^{\it{(vw)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1}
\end{gathered}
%\vspace{-2mm}
\end{equation}   

\begin{equation}
\begin{gathered}
\label{eq:multivideo}
\min_{\bf{Z^{(1)}},\bf{Z^{(2)}},\cdots,\bm{Z^{({m})}}} \underbrace{\sum_{v=1}^{m}\lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F}}_{Reconstruction \ error} + \underbrace{\lambda_s \sum_{v=1}^{m} \lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1}}_{Sparsity} \\ + \underbrace{\lambda_v \sum_{\substack{1\leq v,w\leq m \\ v \neq w}}f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})}_{Diversity} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1},\ {\bf{Z^{(\it{v})}}} \in \mathbb{R}^{n_v\times n_v},\ \forall \ 1 \leq \it{v} \leq m	
\end{gathered}
%	\vspace{-2mm}
\end{equation}   

\begin{equation}
\begin{gathered}
\label{eq:multivideowithonev}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda_s \lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} + \lambda_v \sum_{w=1, v \neq w}^{m}f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}}) \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:diversityall}
\sum_{w=1, v \neq w}^{m}f_{d}({\bf{Z^{(\it{v})}}},\bf{Z^{(\it{w})}})=\sum_{w=1, v \neq w}^{m}\lVert{\bf{W^{\it{(vw)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1} \\ =\lVert{\bf{W^{\it{(v)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:onev1}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda_s \lVert {\bf{Z^{\it{(v)}}}\rVert}_{2,1} + \lambda_v \lVert{\bf{W^{\it{(v)}}}\bf{Z^{(\it{v})}} \rVert}_{2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:onev2}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda \lVert {(\bf{I+W^{\it{(v)}}})\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation} 

\begin{equation}
\begin{gathered}
\label{eq:onev3}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda \lVert {\bf{K^{\it{(v)}}}\bf{Z^{\it{(v)}}}\rVert}_{2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal}
\min_{\bf{Z^{(\it{v})}}}\ \lVert {\bf{X^{\it{(v)}}} - \bf{X^{\it{(v)}}Z^{\it{(v)}}} \rVert}^2_{F} + \lambda \lVert {\bf{Z^{\it{(v)}}}\rVert}_{\textbf{K},2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal2}
\min_{\bf{Z}}\ \lVert {\bf{X} - \bf{X}Z \rVert}^2_{F} + \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1} \\  
s.t.\ \ {\bf{Z^{(\it{v})^{T}}}1 = 1}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal3}
\underline{\min_{\bf{Z}}\ \lVert {\bf{X} - \bf{X}Z \rVert}^2_{F} + \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1}}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:onevfinal4}
\lVert {\bf{X} - \bf{XZ} \rVert}^2_{F}={\lVert {\bf{X}_{\it{original}}} - \bf{X}_{\it{original}}Z \rVert}^2_{F}+\alpha {\lVert \bf{1^{\it{T}}}-\bf{1^{\it{T}}}\bf{Z} \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm1}
\min_{\bf{Z,U}}\ \lVert {\bf{X} - \bf{X}U \rVert}^2_{F} + \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1} \\  
s.t.\ \ {\bf{U=Z}}	
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm2}
{\mathcal{L}_{\mu}(\bf{U,Z,\Lambda})} = \frac{1}{2}\lVert {\bf{X} - \bf{XU} \rVert}^2_{F}+\lambda {\lVert \bf{Z} \rVert}_{\textbf{K},2,1}	+ \langle\mathbf{\Lambda}, \textbf{U}-\textbf{Z}\rangle \\ + \dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z} \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm3}
\min_{\textbf{U}} \ \frac{1}{2}\lVert {\bf{X} - \bf{XU} \rVert}^2_{F}+\langle\mathbf{\Lambda}, \textbf{U}-\textbf{Z}\rangle + \dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z} \rVert}^2_{F} \\
\Leftrightarrow \min_{\textbf{U}} \ \frac{1}{2}\textbf{U}^{T}(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})\textbf{U}-(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})^{T}\textbf{U}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm4}
(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})\textbf{U}=(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm5}
\underline{\textbf{U}=(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})^{-1}(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm6}
\min_{\textbf{Z}} \ \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1}+\langle\mathbf{\Lambda}, \textbf{U}-\textbf{Z}\rangle+\dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z} \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm7}
\min_{\textbf{Z}} \ \lambda \lVert {\bf{Z}\rVert}_{\textbf{K},2,1} + \dfrac{\mu}{2}\lVert {\textbf{U} - \textbf{Z}+\mathbf{\Lambda}/\mu \rVert}^2_{F}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm8}
\min_{\textbf{Z}} \ \sum_{i=1}^{n}\Big [\lambda \textbf{K}_{ii}{\lVert \textbf{Z}_i\rVert}_2+\frac{\mu}{2} {\lVert\textbf{U}_i-\textbf{Z}_i+\frac{1}{\mu}\mathbf{\Lambda}_i \rVert}^2_{F}\Big]
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm9}
\textbf{Z}_i=\max  \Big\{{\lVert r_i \rVert}_2 - \frac{\lambda\textbf{K}_{ii}}{\mu},0\Big\}\frac{r_i}{{\lVert r_i \rVert}_2}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm10}
\underline{\textbf{Z}=Shrink\Big(\textbf{U}+\frac{\mathbf{\Lambda}}{\mu},\frac{\lambda\textbf{K}}{\mu}\Big)= S_{\frac{\lambda\textbf{K}}{\mu}}(\textbf{U}+\mathbf{\Lambda}/\mu)}
\end{gathered}
%	\vspace{-2mm}
\end{equation}

\begin{equation}
\begin{gathered}
\label{eq:admm12}
\underline{\mathbf{\Lambda} \leftarrow \mathbf{\Lambda} + \mu(\textbf{U-Z})}
\end{gathered}
\end{equation}


\begin{equation}
\begin{gathered}
\label{eq:admm13}
(\textbf{X}^{T}\textbf{X}+\mu\textbf{I})^{-1}=\frac{1}{\mu}\textbf{I}-\frac{1}{\mu}\textbf{X}^{T}(\mu\textbf{I}+\textbf{X}\textbf{X}^{T})^{-1}\textbf{X} \\
(\text{Sherman-Morrison-Woodbury formula})
\end{gathered}
\end{equation}


\begin{algorithm} 
	\caption{An ADMM solver for (\ref{eq:onevfinal3})}\label{algo:ADMM}
	\begin{algorithmic}
		\State {\bf Input:} Video feature matrix $\textbf{X}$, $\textbf{K}$ and $\lambda, \mu >0$  
		\While{\textit{not converged}} \\
		\ \ $\textbf{U} \leftarrow (\textbf{X}^{T}\textbf{X}+\mu\textbf{I})^{-1}(\textbf{X}^{T}\textbf{X}+\mu\textbf{Z}-\mathbf{\Lambda})$;\\
		\ \ $\textbf{Z} \leftarrow S_{\frac{\lambda\textbf{K}}{\mu}}(\textbf{U}+\mathbf{\Lambda}/\mu)$ (row-wise);\\
		\ \ $\mathbf{\Lambda} \leftarrow \mathbf{\Lambda} + \mu(\textbf{U-Z})$;
		\EndWhile
		\State {\bf Output:} Sparse coefficient matrix $\textbf{Z}$.
	\end{algorithmic}
\end{algorithm}

%Since the above algorithm computes the exact solutions for each subproblems, its convergence is guaranteed by the existing ADMM theory under mild conditions, following~\cite{glowinski1989augmented}.
%
%{\bf Theorem 1.} \textit{For $\lambda>0$ and $\mu \in (0,\frac{\sqrt{5}+1}{2})$, the sequence generated $(\textbf{U}_{(k)},\textbf{Z}_{(k)})$ by Algo.~\ref{algo:ADMM} from any starting point $(\textbf{U}_{(0)},\textbf{Z}_{(0)})$ monotonically decreases the objective function value and converges to $(\textbf{U}_{(\star)},\textbf{Z}_{(\star)})$, where $(\textbf{U}_{(\star)},\textbf{Z}_{(\star)})$ is a solution of (\ref{eq:onevfinal3}) and $k$ denotes the iteration number}. 

\begin{algorithm} 
	\caption{Algorithm for solving (\ref{eq:multivideo})}\label{algo:OverallALM}
	\begin{algorithmic}
		\State {\bf Input:} Video feature matrices ${\bf{X^{(1)}},\bf{X^{(2)}},\cdots,\bm{X^{({m})}}}$ 
		\For{\textit{each v}} \\
		\ \ Initialize ${\bf{Z^{(\it{v})}}}$ by solving (\ref{eq:naivemultivideo});
		\EndFor
		\While{\textit{not converged}} 
		\ \ \For{\textit{each v}} \\
			\ \ \ \ \ \ \  Obtain ${\bf{Z^{(\it{v})}}}$ by solving (\ref{eq:onevfinal3}); 
		\EndFor
		\EndWhile
		\State {\bf Output:} Coefficient matrices ${\bf{Z^{(1)}},\bf{Z^{(2)}},\cdots,\bm{Z^{({m})}}}$.
	\end{algorithmic}
\end{algorithm}

%{\bf Theorem 2.} \textit{The alternating optimization procedure in solving (\ref{eq:multivideo}) will monotonically decrease the function value and hence guaranteed to converge with Algo.~\ref{algo:OverallALM}.}
%\newline
%\textbf{Proof.}     


  
    


